Multidimensional characterization of particle morphology and mineralogical composition using CT data and R-vine copulas

Computed tomography (CT) can capture volumes large enough to measure a statistically meaningful number of micron-sized particles with a sufficiently good resolution to allow for the analysis of individual particles. However, the development of methods to efficiently investigate such image data and interpretably model the observed particle features is still an active field of research. When image data of particles exhibiting a wide range of shapes and sizes is considered, traditional image segmentation methods, such as the classic watershed algorithm, struggle to recognize particles with satisfying accuracy. Thus, more advanced methods of machine learning must be utilized for image segmentation to improve the validity of subsequent analyzes. Moreover, CT data does not include information about the mineralogical composition of particles and, therefore, additional SEM-EDS image data has to be acquired. In this paper, micro-CT image data of a particle system mostly consisting of zinnwaldite-quartz composites is considered. First, an image segmentation method is applied which uses deep convolutional neural networks, in particular an adaptation of the U-net architecture. This has the advantage of requiring less hand-labeling than other machine learning methods, while also being more flexible with the possibility of transfer learning. Then, fully parameterized models based on vine copulas are designed to determine multivariate probability distributions of descriptor vectors for the size, shape, texture and composition of particles -- allowing for the estimation and interpretable characterization of interdependencies between particle descriptors. For model fitting, the segmented three-dimensional CT data and co-registered two-dimensional SEM-EDS data are used.

==> Figure8.tex <==
\begin{figure}[ht]


\tikzset{every picture/.style={line width=0.75pt}} 

\begin{tikzpicture}[x=0.75pt,y=0.75pt]
\draw (113.08,77.73) node  {\includegraphics[width=139.53pt,height=70.58pt]{pictures/New_Hists/zinIntensity.Mean.pdf}};
\draw (315.52,77.79) node  {\includegraphics[width=139.53pt,height=70.58pt]{pictures/New_Hists/mixIntensity.Mean.pdf}};
\draw (516.41,77.68) node  {\includegraphics[width=139.53pt,height=70.58pt]{pictures/New_Hists/quaIntensity.Mean.pdf}};
\draw (113.65,188.73) node  {\includegraphics[width=139.53pt,height=70.58pt]{pictures/New_Hists/zinIQR.pdf}};
\draw (316.09,188.79) node  {\includegraphics[width=139.53pt,height=70.58pt]{pictures/New_Hists/mixIQR.pdf}};
\draw (516.98,188.68) node  {\includegraphics[width=139.53pt,height=70.58pt]{pictures/New_Hists/quaIQR.pdf}};
\draw (111.08,299.73) node  {\includegraphics[width=139.53pt,height=70.58pt]{zinVolume.png}};
\draw (313.52,299.79) node  {\includegraphics[width=139.53pt,height=70.58pt]{pictures/New_Hists/mixVolume.pdf}};
\draw (514.41,299.68) node  {\includegraphics[width=139.53pt,height=70.58pt]{pictures/New_Hists/quaVolume.pdf}};
\draw (111.65,410.73) node  {\includegraphics[width=139.53pt,height=70.58pt]{pictures/New_Hists/zinSphericity.pdf}};
\draw (314.09,410.79) node  {\includegraphics[width=139.53pt,height=70.58pt]{pictures/New_Hists/mixSphericity.pdf}};
\draw (514.98,410.68) node  {\includegraphics[width=139.53pt,height=70.58pt]{pictures/New_Hists/quaSphericity.pdf}};
\draw (113.65,521.73) node  {\includegraphics[width=139.53pt,height=70.58pt]{pictures/New_Hists/zinFlatness.pdf}};
\draw (316.09,521.79) node  {\includegraphics[width=139.53pt,height=70.58pt]{pictures/New_Hists/mixFlatness.pdf}};
\draw (516.98,521.68) node  {\includegraphics[width=139.53pt,height=70.58pt]{pictures/New_Hists/quaFlatness.pdf}};
\draw (111.08,632.73) node  {\includegraphics[width=139.53pt,height=70.58pt]{pictures/New_Hists/zinElongation.pdf}};
\draw (313.52,632.79) node  {\includegraphics[width=139.53pt,height=70.58pt]{pictures/New_Hists/mixElongation.pdf}};
\draw (514.41,632.68) node  {\includegraphics[width=139.53pt,height=70.58pt]{pictures/New_Hists/quaElongation.pdf}};




\end{tikzpicture}

\caption{Histograms and fitted marginal probability densities of shape, size and texture descriptors of particles predominantly composed of zinnwaldite  (left column) and  quartz   (right column). }
\label{fig:histograms_all}
\end{figure}

==> pictures/table_confusionMatrix.tex <==
\begin{table}[H]
	\centering
    \caption{
    Confusion matrices of the copula-based decision rule given in (\ref{eq:prediction}) for particles observed in the SEM-EDS section which has been used for adjusting the prediction model and for the particles observed in the SEM-EDS section which was withheld for validation. 
    }
	\label{tab:confusionMatrix}
		\begin{tabular} {l | c   c | c c|}
				\cline{2-5}
				& \multicolumn{2}{c}{\bf{calibration section}} \vline & \multicolumn{2}{c|}{\bf{validation section}}\\
				\cline{2-5}
			 	{} & \bf{zinnwaldite} & \bf{quartz} &  \bf{zinnwaldite} & \bf{quartz} \\ \hline 
			 	\multicolumn{1}{ |c | }{ \bf{predicted zinnwaldite}} & 333  & 25 & 204 & 19 \\
			 	\multicolumn{1}{ |c | }{ \bf{predicted quartz}}   & 9 &  437 & 12 & 244\\ \hline		 	
	        \end{tabular}
\end{table}






==> pictures/table_confusionMatrix1D.tex <==
\begin{table}[H]
	\centering
    \caption{Confusion matrix for predicting the particle composition based on one-dimensional densities of the median grayscale value, where the particles observed in the SEM-EDS data have been used for adjusting the prediction model.}
	\label{tab:confusionMatrix1D}
		\begin{tabular} {l | c   c}
		 	{} & \bf{zinnwaldite} & \bf{quartz} \\ \hline \bf{predicted zinnwaldite} & 269  & 26 \\
		 	\bf{predicted quartz} & 73 &  436
        \end{tabular}
\end{table}

==> pictures/table_confusionMatrix2D.tex <==
\begin{table}[H]
	\centering
    \caption{Confusion matrix for predicting the particle composition based on joint densities of the sphericity factor and the median grayscale value, where the particles observed in the SEM-EDS data have been used for adjusting the prediction model.}
	\label{tab:confusionMatrix2D}
		\begin{tabular} {l | c   c}
		 	{} & \bf{zinnwaldite} & \bf{quartz} \\ \hline \bf{predicted zinnwaldite} & 315  & 33 \\
		 	\bf{predicted quartz} & 27 &  429
        \end{tabular}
\end{table}

==> pictures/table_confusionMatrix_lda_copula.tex <==
\begin{table}[H]
	\centering
    \caption{Confusion matrix of the copula-based decision rule utilizing dimension reduction. The corresponding fitted probability densities are visualized in Figures~\ref{fig:lda_pdf}c~and~\ref{fig:lda_pdf}d.}
	\label{tab:confusionMatrix_lda_copula}
		\begin{tabular} {l | c   c | c c|}
			\cline{2-5}
			& \multicolumn{2}{c}{\bf{calibration section}} \vline & \multicolumn{2}{c|}{\bf{validation section}}\\
			\cline{2-5}
		 	{} & \bf{zinnwaldite} & \bf{quartz} &  \bf{zinnwaldite} & \bf{quartz} \\ \hline 
		 	\multicolumn{1}{ |c | }{ \bf{predicted zinnwaldite}} & 323  & 17 & 207 & 8 \\
		 	\multicolumn{1}{ |c | }{ \bf{predicted quartz}}  & 19 &  445 & 9 & 255\\ \hline		 	
        \end{tabular}
\end{table}

==> pictures/table_confusionMatrix_lda_kernel.tex <==
\begin{table}[H]
	\centering
    \caption{Confusion matrix of the decision rule utilizing dimension reduction followed by kernel density estimation. The corresponding probability densities are visualized in Figures~\ref{fig:lda_pdf}a~and~\ref{fig:lda_pdf}b.}
	\label{tab:confusionMatrix_lda_kernel}
		\begin{tabular} {l | c   c | c c|}
			\cline{2-5}
			& \multicolumn{2}{c}{\bf{calibration section}} \vline & \multicolumn{2}{c|}{\bf{validation section}}\\
			\cline{2-5}
		 	{} & \bf{zinnwaldite} & \bf{quartz} &  \bf{zinnwaldite} & \bf{quartz} \\ \hline 
		 	\multicolumn{1}{ |c | }{ \bf{predicted zinnwaldite}} & 331  & 12 & 205 & 8 \\
		 	\multicolumn{1}{ |c | }{ \bf{predicted quartz}}  & 11 &  450 & 11 & 255\\ \hline		 	
        \end{tabular}
\end{table}



==> pictures/table_confusionMatrix_validation.tex <==
\begin{table}[H]
	\centering
    \caption{}
	\label{tab:confusionMatrix_validation}
		\begin{tabular} {l | c   c}
		 	{} & \bf{zinnwaldite} & \bf{quartz} \\ \hline \bf{predicted zinnwaldite} & 204  & 19 \\
		 	\bf{predicted quartz} & 12 &  244
        \end{tabular}
\end{table}

==> pictures/table_corrcoeff_zinnwaldite.tex <==
\begin{table}[H]
	\centering
    \caption{Correlation coefficients of particle characteristics for zinnwaldite.}
	\label{tab:corrcoeff_zinnwaldite}
		\begin{tabular} {l | l |l | l |l | l | l}
			\bf{} & \bf{r} & \bf{s} & \bf{c} & \bf{e} & \bf{m} & \bf{iqr} \\ \hline
       		\bf{r} & 1.0000  &  0.1450 &   0.0695  &  0.3443 &   0.4939 &   0.2825 \\
       		\bf{s} &     0.1450  &  1.0000 &   0.5936  &  0.4400 &   0.3636 &    0.2632 \\
       		\bf{c} &  0.0695 &   0.5936 &   1.0000 &  -0.0663  &  0.3606   & 0.1267\\
       		\bf{e} &     0.3443  &  0.4400 &  -0.0663 &   1.0000  &  0.2155 &   0.2771\\
       		\bf{m} &     0.4939 &   0.3636 &   0.3606  &  0.2155 &   1.0000  &  0.2276\\
       		 \bf{iqr} &    0.2825  &  0.2632  &  0.1267  &  0.2771  &  0.2276 &   1.0000\\       		
        \end{tabular}
\end{table}


==> pictures/table_parameters_zinn.tex <==
\begin{table}[H]
	\centering
    \caption{Parameters of fitted distributions.}
	\label{tab:parameters_zinn}
		\begin{tabular} {l | l |l | l}
			\bf{characteristic} & \bf{distribution} & \bf{zinnwaldite} & \bf{quartz} \\ \hline
            volume equivalent radius & gamma & $k=7.16, \theta=6.84$ & $k=6.84, \theta=9.8$ \\
			sphericity factor & beta & $\alpha = 7.17   , \beta = 7.05 $ & $\alpha = 10.73, \beta = 4.63 $ \\
			convexity factor  & beta & $\alpha = 12.61, \beta = 2.97$    & $\alpha = 17.35, \beta = 2.73$   \\
			elongation factor & beta & $\alpha = 2.00, \beta = 4.73$ & $\alpha = 2.90, \beta =  2.74$ \\
			median grayscale value & beta &  $\alpha =   14.12, \beta = 18.32$&  $\alpha =  74.95, \beta = 166.85$\\
			interquartile range & beta & $\alpha = 3.78, \beta = 38.54$ & $\alpha = 4.52, \beta = 112.11$

        \end{tabular}
\end{table}
